More connection, less community: network formation and local public goods provision

This paper presents a model of network formation and public goods provision in local communities. Here, networks can sustain public good provision by spreading information about people's behaviour. I find a critical threshold in network connectedness at which public good provision drops sharply, even though agents are highly heterogeneous. Technology change can tear a community's social fabric by pushing high-skilled workers to withdraw from their local community. This can help explain rising resentment toward perceived ``elites'' -- their withdrawal actively harms those left behind. Moreover, well-meaning policies that upskill workers can make them worse off by reducing network connectedness.

==> A.notation_list.tex <==
%\begin{table}
%\caption{Variables in the main model}
%\centering
\begin{longtable}{p{0.15\textwidth} p{0.25\textwidth} >{\centering\arraybackslash}p{0.55\textwidth}}  
Variable        & Space             & Description \\
\hline
\multicolumn{3}{c}{Agents} \\
\hline
$n$             & $\mathbb{Z}^+$   & Number of agents \\
$i,j,\ell$      & $\{1,...,N\}$     & Typical agents \\
\hline
\multicolumn{3}{c}{Decisions} \\
\hline
$t_i$           & $[0,1]$           & Time $i$ spends inside community  \\
$t_i^{out}$     & $[0,1]$           & Time $i$ spends outside community  \\
$x_i$           & $\{0,1\}$         & $i$'s public good provision \\
\hline
\multicolumn{3}{c}{Social network} \\
\hline
$d_i$           & $\{0,...,D\}$     & $i$'s degree  \\
$D$             & $\mathbb{Z}^+$    & Maximum possible degree (no. of friends)  \\
$p(d|t_i)$      & $p:\mathbb{R} \to [0,1]$  & PMF \\
$P(d_i = d | t_i)$ & $[0,1]$        & Probability \\
$\mathbf{d} = (d_i)_{i=1}^n$ & $(d_1,...,d_n)$   & Degree distribution \\
$\mathcal{G}((d_i)_{i=1}^n)$ &      & Configuration model \\
$G^{(n)}$       & $n \times n$ matrix & Realisation of $\mathcal{G}((d_i)_{i=1}^N$ \\
$\lambda_d$     & $[0,1]$           & Fraction of agents with degree $d$ \\
\hline
\multicolumn{3}{c}{Observation \& Reward networks} \\
\hline
$\mathcal{N}_i^o$ / $\mathcal{N}_i^r$ &  & set of observers / rewarders \\
$d_i^o$ / $d_i^r$  & $\mathbb{Z}^+$   & no. of observers / rewarders \\
$k_i^o$ / $k_i^r$  & $\mathbb{R}^+$   & constant governing no. of observers / rewarders \\
$a$             & $(0, \frac{1}{6})$ & exponent governing no. of observers/rewarders \\
\hline
\multicolumn{3}{c}{Preferences} \\
\hline
$C_i$           & $\mathbb{R}^+$    & Marginal cost of providing public goods \\
$R$             & $\mathbb{R}^+$    & Size of reward \\
$p_i(\text{reward})$ & $[0,1]$      & Probability of receiving reward \\
$\pi$           & $\mathbb{R}^+$     & Benefit of interaction inside community \\
$\pi^{out}$     & $\mathbb{R}^+$     & Benefit of interaction outside community \\
$F(\cdot)$      & $F: \mathbb{R} \to [0,1]$ & CDF of cost parameters \\
$B(\cdot)$      & $B: [0,1] \to \mathbb{R}$ & Benefits from others' public good provision \\
$c(\cdot)$      & $c: \mathbb{R}^+ \to \mathbb{R}^+$ & Cost of total time \\
$I(\cdot)$      & $I: [0,1] \to \mathbb{R}$ & No. interactions inside \\
$I_{out}(\cdot)$& $I_{out}: [0,1] \to \mathbb{R}$ & No. interactions outside \\
$v_i$           & $v_i: \mathbb{R} \to \mathbb{R}$ & Second stage utility function \\
$u_i$           & $u_i: \mathbb{R} \to \mathbb{R}$ & Overall utility function \\
\hline
\multicolumn{3}{c}{Other} \\
\hline
$S$             & $[0,1]$           & Level of public good provision \\
$\mu$           & $(0.5,1)$         & a number \\
$w_i := u_i - v_i$ & $w_i: \mathbb{R} \to \mathbb{R}$ & `direct' first stage payoffs \\
$\hat{t}$ / $\hat{t}^{out}$ & $[0,1]$ & maximiser of $w_i$ \\
\end{longtable}
%\end{table}


\subsection*{Extension}
{\setlength{\extrarowheight}{3pt}%
\begin{longtable}{b{0.15\textwidth} b{0.25\textwidth} >{\centering\arraybackslash}b{0.55\textwidth}}  
Variable        & Space             & Description \\
\hline
\multicolumn{3}{c}{Households} \\
\hline
$H$             & $\mathbb{Z}^+$   & Number of households \\
$h$             & $\{1,...,H\}$     & Typical household \\
\hline
\multicolumn{3}{c}{Decisions} \\
\hline
$t_i^{int}$     & $[0,1]$           & initial choice of $t_i$  \\
$t_i^{opt}$     & $[0,1]$           & optimal choice if $i$ chose $t_h$ directly \\ 
$t_h$           & $[0,1]$           & time household $h$ spends in community  \\
$\Tilde{t}^{out}(\cdot)$ & $\Tilde{t}^{out}: [0,1] \to [0,1]$ & optimal $t_i^{out}$ for a given $t_i$ \\
$t_h^{crit}$ & $\mathbb{R}$ & min $t_h$ needed for $P_{SC} = 1$ \\
$t_h^{uncrit}$ & $\mathbb{R}$ & max $t_h$ for $P_{SC} = 0$ \\
$t^{max}$ & $[0,1]$ & max time $i$ is willing to spend in community to get high public good provision \\
\hline
\multicolumn{3}{c}{Social network} \\
\hline
$\xi$           & $[-\Bar{\xi}, \Bar{\xi}]$ & Size of `friendship shock' \\
$\Bar{\xi}$     & $\mathbb{R}^+$    & Maximum size of shock \\
$P_{SC}$        & $[0,1]$       & Probability of `high' public goods (after shock $\xi$) \\
$\hat{F}(\cdot)$& $\hat{F}: \mathbb{R} \to [0,1]$ & CDF of $\xi$, for $\Bar{\xi} = 1$ \\
$\hat{F}_{\Bar{\xi}}(\cdot)$ & $\hat{F}_{\Bar{\xi}}: \mathbb{R} \to [0,1]$ & CDF of $\xi$ \\
$\Tilde{d}_i$   & $\mathbb{Z}^+$    & No. of friends after shock \\
\hline
\multicolumn{3}{c}{Other} \\
\hline
$f(\cdot)$ & $f:[0,1] \to \mathbb{R}$ & an increasing function \\
$z$ & $\mathbb{R}$ & a placeholder \\
\hline
\end{longtable}  }


==> B3.proof_coord_ext.tex <==
\subsection*{Building towards Remark 5} %\Cref{rem:best_response}
To prove \Cref{rem:best_response}, it is helpful to state a pair of lemmas. The first shows that the critical threshold of network connectivity (that we found in \Cref{prop:main_result}) can be expressed as a function of the households' choices of $t_h$, plus the shock $\xi$. The second shows critical values of $t_h$ that ensure the network connectivity is definitely (i.e.. with probability 1) above, and definitely below, the threshold. And it shows that the difference between these two values shrinks to zero as $\Bar{\xi} \to 0$, and hence that the gradient of the utility function between the two values becomes large.\footnote{The important feature is that the gradient is positive, rather than large.}

\subsubsection*{First Lemma}
\begin{lem}\label{lem:technical_3}
    For some strictly increasing function $f(\cdot)$, and positive constant $k$:
    \begin{align}
        \lim_{n \to \infty} \frac{1}{n} \sum_{i=1}^n \tilde{d}_i (\tilde{d_i} - 2) = \sum_d d(d-2) \Tilde{\lambda}_d = \frac{1}{H} \sum_{h=1}^H f(t_h) + \xi k.
    \end{align}
\end{lem}

\noindent \emph{Proof.} \\ 

By definition, we have $\tilde{d}_i = d_i$ for all agents not affected by the shock. For those affected by the shock we have $\tilde{d}_i = d_i + 1$ if $\xi > 0$ and $\tilde{d}_i = d_i - 1$ if $\xi < 0$. Define $\Xi := \{i : i \text{ affected by shock}\}$. And by definition, $n^{-1} \cdot |\Xi| = \xi$. Therefore when $\xi > 0$:

\begin{align}
    \frac{1}{n} \sum_i \Tilde{d}_i (\Tilde{d}_i - 2) 
    &= \frac{1}{n} \sum_{i \ \notin \ \Xi} d_i (d_i - 2) + \sum_{i \ \in \ \Xi} (d_i + 1) (d_i - 1) \\
    &= \frac{1}{n} \sum_{i = 1}^n d_i (d_i - 2) + \frac{1}{n} \sum_{i \ \in \ \Xi} (2 d_i - 1) \\
    \lim_{n \to \infty} \frac{1}{n} \sum_i \Tilde{d}_i (\Tilde{d}_i - 2) &= \lim_{n \to \infty} \frac{1}{n} \sum_{i = 1}^n d_i (d_i - 2) + \xi (2 \bar{d} - 1)
\end{align}
where $\bar{d} := \frac{1}{|\Xi|} \sum_{i \in \Xi} d_i$. And when $\xi < 0$:
\begin{align}
    \frac{1}{n} \sum_i \Tilde{d}_i (\Tilde{d}_i - 2) 
    &= \frac{1}{n} \sum_{i \ \notin \ \Xi} d_i (d_i - 2) + \sum_{i \ \in \ \Xi} (d_i - 1) (d_i - 3) \\
    &= \frac{1}{n} \sum_{i = 1}^n d_i (d_i - 2) - \frac{1}{n} \sum_{i \ \in \ \Xi} (2 d_i - 3) \\
   \lim_{n \to \infty} \frac{1}{n} \sum_i \Tilde{d}_i (\Tilde{d}_i - 2) &= \lim_{n \to \infty} \frac{1}{n} \sum_{i = 1}^n d_i (d_i - 2) + \xi (2 \bar{d} - 3)
\end{align}
Note that our assumption that the shock only hits people who have $d_i \geq 2$ means that $(2 \bar{d} - 1) > (2 \bar{d} - 3) > 0$. So we let $k = (2 \bar{d} - 1) > 0$ if $\xi >0$ and $k= (2 \bar{d} - 3) > 0$ if $\xi < 0$. Then we can do some work on the first of the RHS terms. First, we can re-express the average in terms of the fraction of agents with each degree $d$, and then break this down into the `contribution' from each household $h$.
\begin{align}
    \lim_{n \to \infty} \frac{1}{n} \sum_{i=1}^n d_i (d_i - 2) 
    &= \sum_{d=0}^{D} d (d - 2) \lambda_d \\
    &= \frac{1}{H} \sum_h \sum_{d=0}^{D} d (d - 2) p_h(d | t_h)
\end{align}
where $p_h(d | t_h) = P(d_i = d | t_h)$. Note that in household $h$, the fraction of agents with degree $d_i = d$ converges to the probability that a randomly selected agent has that degree. There are two steps to see this. First, all agents $i \in h$ have the same choice of $t_i$ by assumption, and so their degrees are random draws from the same distribution. Second, as $n \to \infty$, the number of agents in household $h$ also grows large, so a Law of Large Numbers applies.
So for each household, this is simply the second moment of the distribution $p_h(d|t_h)$ minus twice the first moment. And we have assumed that this is an increasing function of $t_h$---which we can write as $f(t_h)$. This is a variant of \Cref{lem:threshold_t_hat}, but for each household separately.
%
Putting this all together yields
\begin{align}
    \lim_{n \to \infty} \frac{1}{n} \sum_i \Tilde{d}_i (\Tilde{d}_i - 2) 
    &= \frac{1}{H} \sum_h f(t_h) + k \xi
\end{align}
\hfill $\square$ 

We now need to define the probability of being above the critical threshold. Let
\begin{align}
    P_{SC} := Pr \left( \lim_{n \to \infty} \frac{1}{n} \sum_{i=1}^n \tilde{d}_i (\tilde{d_i} - 2) > 0 \right).
\end{align}

\subsubsection*{Second Lemma} %(\Cref{lem:technical_4}) 
\begin{lem}\label{lem:technical_4}
For any $\Bar{\xi} > 0$: 

(i) \ \ there is a unique $t^{crit}_h := t^{crit}(t_{-h})$ such that $P_{SC} = 1$ for all $t_h \geq t^{crit}_h$,

(ii) \ there is a unique $t^{uncrit}_h := t^{uncrit}(t_{-h})$ such that $P_{SC} = 0$ for all $t_h \leq t^{uncrit}_h$,

(iii) $\frac{d P_{SC}}{d t_h} > 0$ whenever $t_h \in [t^{uncrit}_h, t^{crit}_h]$.

\noindent As $\Bar{\xi} \to 0$:

(iv) \ $\frac{d P_{SC}}{d t_h} \to \infty$ for $t_h \in [t^{uncrit}_h, t^{crit}_h]$,

(v) \ \ $(t^{crit}_h - t^{uncrit}_h) \to 0^+$.
\end{lem}

\noindent \emph{Proof.} \\

It follows from \Cref{prop:main_result} that public good provision is high \emph{with high probability} if and only if $\frac{1}{n} \sum_i \Tilde{d}_i (\Tilde{d}_i - 2) > 0$, where $(\Tilde{d}_i)_{i=1}^n$ is the post-shock degree distribution. Therefore, $P_{SC} = Pr(\lim_{n \to \infty} \frac{1}{n} \sum_i \Tilde{d}_i (\Tilde{d}_i - 2) > 0)$. Using \Cref{lem:technical_3}, we can write 
\begin{align}
    P_{SC} &= Pr \left(\lim_{n \to \infty}  \frac{1}{n} \sum_i \Tilde{d}_i (\Tilde{d}_i - 2) > 0 \right) \\
    &= Pr \left(\frac{1}{H} \sum_h f(t_h) + \xi k > 0 \right).
\end{align}
Then simply rearrange terms, apply the CDF in the standard way, and finally apply the relationship we assumed between $\hat{F}(z)$ and $\hat{F}_{\Bar{\xi}}(z)$.
\begin{align}
    \lim_{n \to \infty} P_{SC} &= P \left(\xi > - \frac{1}{H}\sum_h f(t_h) k^{-1}  \right) \\
    &= 1 - P \left(\xi < - \frac{1}{H}\sum_h f(t_h) k^{-1}  \right) \\
    &= 1 - \hat{F}_{\bar{\xi}}\left(- \frac{1}{H}\sum_h f(t_h) k^{-1}  \right) \\
    &= 1 - \hat{F}\left(- \frac{1}{\bar{\xi}} \frac{1}{H} \frac{1}{k} \sum_h f(t_h)  \right)
\end{align}

Now by the definition of $\hat{F}(\cdot)$, we have $P_{SC} = 1$ whenever
\begin{align}
    %- \frac{1}{\bar{\xi}} \frac{1}{H} \frac{1}{k} \sum_h f_h(t_h) &\leq -1 \\
    \frac{1}{H} \frac{1}{k} \sum_h f(t_h) &\geq \Bar{\xi}.
\end{align}
Consider some household $h'$ and fix $t_h$ for all $h \neq h'$. Then we have $P_{SC} = 1$ whenever
\begin{align}\label{eq:t_crit_defn}
    f(t_{h'}) \geq \Bar{\xi} H k - \sum_{h \neq h'} f(t_h)
\end{align}

Since $f(t_{h'})$ is a strictly increasing function, and $f(t_{h'}) = 0$ for some $t_{h'} \in (0,1)$, then there must be a unique value of $t_{h'}$ that satisfies \cref{eq:t_crit_defn} with equality. Denote this value $t_{h'}^{crit}$. It is a function of all other $t_h$'s; $t_{h'}^{crit} = t^{crit}(t_{-h})$. Note however, that there is absolutely no guarantee that this value is feasible (i.e. it is on the $[0,1]$ interval and so is something that household $h'$ could actually choose). \textbf{This proves part (i).} \\

And similarly we have $P_{SC} = 0$ whenever
\begin{align}
    %- \frac{1}{\bar{\xi}} \frac{1}{H} \frac{1}{k} \sum_h f_h(t_h) &\geq 1 \\
    \frac{1}{H} \frac{1}{k} \sum_h f(t_h) &\leq - \Bar{\xi}.  
\end{align}
Consider some household $h'$ and fix $t_h$ for all $h \neq h'$. Then we have $P_{SC} = 0$ whenever
\begin{align}\label{eq:t_uncrit_defn}
    f(t_{h'}) \leq -\Bar{\xi} H k - \sum_{h \neq h'} f(t_h)
\end{align}
Since $f(t_{h'})$ is a strictly increasing function, and $f(t_{h'}) = 0$ for some $t_{h'} \in (0,1)$, then there must be a unique value of $t_{h'}$ that satisfies \cref{eq:t_uncrit_defn} with equality. Denote this value $t_{h'}^{uncrit}$. It is a function of all other $t_h$'s; $t_{h'}^{uncrit} = t^{uncrit}(t_{-h})$. Again, there is absolutely no guarantee that this value is feasible (i.e. it is on the $[0,1]$ interval and so is something that household $h'$ could actually choose). \textbf{This proves part (ii).} \\

Given this, we have:
\begin{align}
    \text{For } t_{h'} \notin [f(t^{uncrit}_{h'}), f(t^{crit}_{h'})],& \text{ we have } \frac{d P_{SC}}{d t_{h'}} = 0 \\
    \text{For } t_{h'} \in [f(t^{uncrit}_{h'}), f(t^{crit}_{h'})],& \text{ we have } \frac{d P_{SC}}{d t_{h'}} = \hat{F}'(\cdot) \frac{1}{\bar{\xi}} \frac{1}{H} \frac{1}{k} f'(t_{h'})
\end{align}
Notice that all components of $d P_{SC} / d t_{h'}$ when $t_{h'} \in [f_{h'}(t^{uncrit}_{h'}), f_{h'}(t^{crit}_{h'})]$ are strictly positive (all but $f'_{h'}(\cdot) > 0$ are by assumption). \textbf{This proves part (iii).} And all are finite. But $1/ \Bar{\xi} \to \infty$ as $\Bar{\xi} \to 0$. Therefore when $t_{h'} \in [f_{h'}(t^{uncrit}_{h'}), f_{h'}(t^{crit}_{h'})]$, we have $d P_{SC} / d t_{h'} \to \infty$ as $\bar{\xi} \to 0$. \textbf{This proves part (iv).}

Finally, $t_{h'}^{crit}$ are defined such that they solve $t_{h'}^{uncrit}$ \cref{eq:t_crit_defn} and \cref{eq:t_uncrit_defn} respectively. Therefore we have 
\begin{align}
    f(t_{h'}^{crit}) - f(t_{h'}^{uncrit}) 
    &= \left( \Bar{\xi} H k - \sum_{h \neq h'} f(t_h) \right) - \left( - \Bar{\xi} H k - \sum_{h \neq h'} f(t_h) \right) \\
    &= 2 \Bar{\xi} H k \\
    f(t_{h'}^{crit}) - f(t_{h'}^{uncrit}) &\to 0 \text{ as } \Bar{\xi} \to 0
\end{align}
\textbf{This proves part (v)} and completes the proof. \hfill $\square$


\subsection*{Proof of Remark 5} % (\ref{rem:best_response})
The utility function of a head of household can be written as:
\begin{align}
    \lim_{n \to \infty} u_i = W_i(t_h) + P_{SC} \cdot \Delta v + B(F(0))
\end{align}
It follows from \Cref{lem:technical_4} that:
\begin{align}\label{eq:utility_derivative}
    \frac{d \lim_{n \to \infty} u_i}{d t_h} = 
    \begin{cases}
        \to \infty \text{ as } \bar{\xi} \to 0 &\text{ for } t_h \in [t^{uncrit}, t^{crit}), \\
        \frac{d W_i(t_h)}{d t_h} &\text{ otherwise. }   
    \end{cases}
\end{align}

Therefore the utility function is as shown in \Cref{fig:1_NEW} (panels (B)-(D)). The best responses follow immediately from inspection of the figure. \hfill $\square$ 


\subsection*{Proof of Proposition 3} %  (\Cref{prop:eqm_formation})
The result follows from the discussion that precedes it in the main text. \hfill $\square$


\subsection*{Proof of Remark 6} %(\Cref{prop:comp_stat_formation})
Comparative statics for $\hat{t}$ are covered by the proof to \Cref{rem:comp_statics}. This is because $\hat{t}$ is defined as the maximum of $w_i$, which is unaffected by allowing agents to coordinate. 
For proving the comparative static for $t^{max}$ we use $W(t)$ and its properties, as defined in \Cref{prop:2}. And we use the definition of $\Delta v_i$ from \Cref{defn:t_max}.

\paragraph{$t_i$-max.} By definition, moving from $\hat{t}$ to $t^{max}_i$ causes $W(\cdot)$ to fall by exactly $\Delta v_i$ units (this is from \Cref{defn:t_max}): $W(t^{max}_i | \pi, \pi^{out}) - W(\hat{t} | \pi, \pi^{out}) = \Delta v_i$. And in this range, we know $W'(t | \pi, \pi^{out}) < 0$.

Again, we then know from above that $W'(\cdot)$ decreases when $\pi$ increases and when $\pi^{out}$ increases. So we have $W'(t | \pi_{new}, \pi^{out}_{new}) < W'(t | \pi, \pi^{out})$ for all $t$. In the range $[\hat{t}, t^{max}_i]$, both $W(t | \pi_{new}, \pi^{out}_{new})$ and $W(t | \pi, \pi^{out})$ are decreasing (the second by construction, and the first must be because its maximum point is to the left of that for the second). 

But $W(t | \pi_{new}, \pi^{out}_{new})$ is `steeper' (i.e. its gradient is more negative). So it must be that $W(t^{max}_i | \pi_{new}, \pi^{out}_{new}) - W(\hat{t} | \pi_{new}, \pi^{out}_{new}) > \Delta v_i$. And additionally, $\hat{t}$ is not the maximum point with these new parameter values. So there must also be some fall between $\hat{t}_{new}$ (which is $< \hat{t}$) and $\hat{t}$. That is; $W(\hat{t}_{new} | \pi_{new}, \pi^{out}_{new}) - W(\hat{t} | \pi_{new}, \pi^{out}_{new}) = \epsilon > 0$.

So the move from $\hat{t}_{new}$ to $t^{max}_i$ with the new parameters $\pi_{new}$ and $\pi^{out}_{new}$ must entail a drop of \emph{more than} $A$ units. By the definition of $t^{max}_{new}$ and the continuity of $W(\cdot)$, it must therefore be that $t^{max}_{i, new} < t^{max}$. Put simply: if moving $t^{max}_i - \hat{t}_{new}$ units along a downwards sloping curve causes a fall of more than $\Delta v_i$ units, then we must move fewer than $t^{max}_i - \hat{t}_{new}$ units along that same curve to get a fall of exactly $\Delta v_i$ units.

\paragraph{$t$-max.} By definition, $t^{max}_h = \min_{i \in h} t^{max}_i$. So if $t^{max}_i$ is increasing in $\pi$ and decreasing in $\pi^{out}$ for all $i$, then $t^{max}_h$ must also be increasing in $\pi$ and decreasing in $\pi^{out}$ for all $h$. Finally, recall that $t^{max}_h$ is the same for all $h$ (because we assumed $\Delta v_i = B(F(R)) - B(F(0))$ (i.e. as small as possible) for at least one $i \in h$, for all $h$). Therefore, the result trivially applies to $t^{max} = t^{max}_h$.  \hfill $\square$

%\subsection{Proof of Corollary 2 (\Cref{cor:comp_stat_formation})}
%Follows straightforwardly from \Cref{prop:comp_stat_formation} and the best response function found in \Cref{rem:best_response}.


==> figure_tex_code/figure_1.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.45\textwidth}
        \centering
        %\includegraphics[width=\linewidth]{figures/Fig_1A.jpg}
        \includegraphics[width=\linewidth]{figures/Figure_1A.png}
        %\vspace{13mm}
        \caption{}
        \label{fig:1A}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.45\textwidth}
        \centering
        %\includegraphics[width=\linewidth]{figures/Fig_1B.jpg}
        \includegraphics[width=\linewidth]{figures/Figure_1B.png}
        %\vspace{3mm}
        \caption{}
        \label{fig:1B}
    \end{subfigure}

    \caption{(A) Optimal choice of $t_i^{out}$ for given values of $t_i$. Green line has $t_i = t_3$. Yellow line has $t_i = 2$. Purple line has $t_i = t_1$. With $t_3 > t_2 > t_1$. (B) An agent's payoffs as a function of $t_i$, assuming optimal choice of $t_i^{out}$: with (blue line) and without social capital (green line).}
    \label{fig:1}
\end{figure}

==> figure_tex_code/figure_2.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering
        \hspace{-18mm}
        %\includegraphics[width=\linewidth]{figures/Fig_2A.jpg}
        \includegraphics[width=1.1\linewidth]{figures/Figure_2A.png}
        %\vspace{3mm}
        \caption{}
        \label{fig:2A}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.3\textwidth}
        \centering
        \hspace{-10mm}
        %\includegraphics[width=\linewidth]{figures/Fig_2B.jpg}
        \includegraphics[width=1.1\linewidth]{figures/Figure_2B.png}
        %\vspace{3mm}
        \caption{}
        \label{fig:2B}
    \end{subfigure}
    %\hfill
    \begin{subfigure}{0.3\textwidth}
        \centering
        \hspace{10mm}
        %\includegraphics[width=\linewidth]{figures/Fig_2C.jpg}
        \includegraphics[width=1.1\linewidth]{figures/Figure_2C.png}
        %\vspace{3mm}
        \caption{}
        \label{fig:2C}
    \end{subfigure}
    \caption{Red line shows utility function assuming optimal choice of $t_i^{out}$. Blue line [resp. green line] shows payoffs with [resp. without] social capital. Panel (A): $t^{crit} < \hat{t}$. Panel (B): $t^{crit} \in [\hat{t}, t^{max}]$. Panel (C): $t^{crit} > t^{max}$.}
    \label{fig:2}
\end{figure}

==> figure_tex_code/figure_2_alt.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        %\includegraphics[width=\textwidth]{figures/Fig_2A.jpg} 
        \includegraphics[width=\textwidth]{figures/Figure_2A.png} 
        \caption{}
        \label{fig:2A}
        \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        %\includegraphics[width=\textwidth]{figures/Fig_2B.jpg}  
        \includegraphics[width=\textwidth]{figures/Figure_2B.png}
        \caption{}
        \label{fig:2B}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        %\includegraphics[width=\textwidth]{figures/Fig_2C.jpg} 
        \includegraphics[width=\textwidth]{figures/Figure_2C.png}
        \caption{}
        \label{fig:2C}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        %\includegraphics[width=\textwidth]{figures/...}
        %\caption{}
        %\label{fig:4D}
    \end{subfigure}
    \caption{Red line shows utility function assuming optimal choice of $t_i^{out}$. Blue line [resp. green line] shows payoffs with [resp. without] social capital. Panel (A): $t^{crit}_h < \hat{t}$. Panel (B): $t^{crit}_h \in [\hat{t}, t^{max}]$. Panel (C): $t^{crit}_h > t^{max}$.}
    \label{fig:2}
\end{figure}

==> figure_tex_code/figure_3.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        %\includegraphics[width=\textwidth]{figures/Fig_3A.jpg}  
        \includegraphics[width=\textwidth]{figures/Figure_3A.png}  
        \caption{}
        \label{fig:3A}
        \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        %\includegraphics[width=\textwidth]{figures/Fig_3B.jpg}
        \includegraphics[width=\textwidth]{figures/Figure_3B.png}
        \caption{}
        \label{fig:3B}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        %\includegraphics[width=\textwidth]{figures/Fig_3C.jpg}
        \includegraphics[width=\textwidth]{figures/Figure_3C.png}
        \caption{}
        \label{fig:3C}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        %\includegraphics[width=\textwidth]{figures/Fig_3D.jpg}
        \includegraphics[width=\textwidth]{figures/Figure_3D.png}
        \caption{}
        \label{fig:3D}
    \end{subfigure}
    \caption{Green line shows Best Response function, purple line shows $t^{crit}(t)$. Orange circles show equilibria. Panel (A) shows unique `friendly' equilibrium. Panel (B) shows `pressured' equilibrium. Panel (C) shows both `pressured' and `unfriendly' equilibria. Panel (D) shows unique `unfriendly' equilibrium. Note that these graphs only show the symmetric equilibria: for each symmetric `pressured' equilibrium, there exists a set of asymmetric ones. `Friendly' and `unfriendly' equilibria are always symmetric.} 
    \label{fig:3}
\end{figure}

==> figure_tex_code/figure_4.tex <==
\begin{figure}[ht!]
    \centering
    \begin{subfigure}[b]{0.475\textwidth}
        \centering
        %\includegraphics[width=\textwidth]{figures/Fig_4A.jpg} 
        \includegraphics[width=\textwidth]{figures/Figure_4A.png} 
        \caption{}
        \label{fig:4A}
        \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}  
        \centering 
        %\includegraphics[width=\textwidth]{figures/Fig_4B.jpg}  
        \includegraphics[width=\textwidth]{figures/Figure_4B.png}
        \caption{}
        \label{fig:4B}
    \end{subfigure}
    \vskip\baselineskip
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        %\includegraphics[width=\textwidth]{figures/Fig_4C.jpg} 
        \includegraphics[width=\textwidth]{figures/Figure_4C.png}
        \caption{}
        \label{fig:4C}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.475\textwidth}   
        \centering 
        %\includegraphics[width=\textwidth]{figures/...}
        %\caption{}
        %\label{fig:4D}
    \end{subfigure}
    \caption{An improvement in technology shifts $\hat{t}$ and $t^{max}$ downwards to $\hat{t}_n$ and $t^{max}_n$ respectively. Panels (A) - (C) show successive technology changes. Blue dashed line is $t^{crit}(t)$. Green line is $BR_i(t)$, given $\hat{t}, t^{max}$. Gray line is $BR_i(t)$, given $\hat{t}_n, t^{max}_n$. Panel (A) shows the shift from a unique friendly equilibrium to a setting with both pressured and unfriendly equilibria. Panel (B) shows a shift that keeps both pressured and unfriendly equilibria, but leads to a change in equilibrium selection. Panel (C) shows the shift to a unique unfriendly equilibrium.} 
    \label{fig:4}
\end{figure}

==> figure_tex_code/figure_5.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/Fig_5.jpg}
    \caption{Welfare}
    \label{fig:5}
\end{figure}

==> figure_tex_code/figure_6.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/Fig_6.jpg}
    \caption{Welfare: internalising the externality}
    \label{fig:6}
\end{figure}

==> literature.tex <==
\subsection{To Read}
\begin{itemize}
    \item \cite{siisiainen2003two} -- an explanation of Putnam vs Bourdieu views of social capital.
    \item \cite{simmel1950sociology} -- this is a book. just dip into a few parts
    \item \cite{karlan2009trust}
    \item \cite{ambrus2014consumption}
    \item \cite{haag2006social}
    \item \cite{ali2022communication}
    \item \cite{markus2009repeated} -- not really relevant; just skim 
    \item \cite{buldyrev2010catastrophic}
\end{itemize}

\subsection{Hard Copy}
\begin{itemize}
    \item \cite{jackson2012social}
    \item \cite{nava2014efficiency}
    \item \cite{wolitzky2013cooperation}
\end{itemize}

\subsection{Social capital: economics}
\begin{itemize}
    \item  \cite{sobel2002can}
    \item \cite{glaeser2002economic} 
    \item \cite{kandori1992social}
    \item \cite{vega2006building}
    \item \cite{ellison1994cooperation}
    \item \cite{ali2016ostracism}
    \item \cite{guiso2006does}
    \item \cite{guiso2011civic}
\end{itemize}

\subsection{Social capital: sociology}
\begin{itemize}
    \item \cite{coleman1988social}
    \item \cite{bourdieu2018forms}
    \item \cite{krackhardt1996social}
\end{itemize}

\subsection{Networks: other}
\begin{itemize}
    \item \cite{gagnon2017networks}: thinks about interactions between market actions and network actions, with a fixed network structure. Then cores of networks matter. \emph{might be possible to riff on this, by saying that people choose between spending time building markets and building networks. Basically, move to an endogenous network.}
\end{itemize}

\subsection{Altruism}
\begin{itemize}
    \item \cite{feigin2014theories}: a review article on different theories of altruism. (1) there is no mention of actions driving altruism. (2) `pseudo-altruism' is a leading theory -- this is the idea that people do nice things because it benefits themselves egoistically. But this is far wider than standard money payoffs; it includes `internal rewards' such as feeling good about oneself. Another similar reason is `arousal reduction': basically avoiding feelings of guilt, shame or unease. \emph{Approx. 200-400 cites}.\footnote{Oddly, the paper is published in two different journals.}

    \item \cite{lay2015altruism}: looks at prosocial behaviour (roughly, this is `being nice'). Main reasons are: altruism, empathy, kin selection. Article is a bit thin. Not super useful. \emph{Approx. 80 cites.}

    \item \cite{batson2003altruism}: `prosocial' is the actual behaviour that helps others, `altruism' is the motivation for helping others.

    \emph{``In the 1960s, heightened social conscience focused attention on anomalous failures to act prosocially. In the broader sweep of Western thought, this focus is itself anomalous. Through the centuries, the puzzle that has intrigued those contemplating the human condition has not been why people fail to care for others in need; the puzzle has been why people care. From Aristotle and Aquinas through Hobbes and Bentham to Nietzsche and Freud, the dominant view in Western thought has been that people are, at heart, exclusively self-interested. Given this view, what explains the enormous effort and energy directed toward benefiting others? ''}

    An interesting philosophical point: the claim that `altruism is just another form of egoism because if people enjoy helping others, then it's just egoistic' has been debunked by philosophers. It confuses different forms of psychological hedonism (p.474).

    The most frequent hypothesis for altruism is \emph{empathy}. Empathy evokes emotions which create motivation for helping others. This argument has been made by Thomas Aquinas, David Hume, Adam Smith, Charles Darwin, Herbert Spencer, and William McDougall, as well as in contemporary psychology by Hoffman (1975), Krebs (1975), and Batson (1987). But this doesn't tell use whether the underlying motivation is altruistic, or about gaining more self-benefits later on.

    ``Most frequently proposed egoistic explanation of the empathy-helping relationship is \emph{aversive-arousal reduction}'. Basically, the claim is that it's unpleasant to feel empathy towards people who are suffering, so helping others is about reducing this unpleasant feeling in oneself. This is very much what economists would call altruism...

    Nevertheless, experiments tend to be consistent with the empathy-altruism hypothesis, rather than the aversive-arousal reduction hypothesis. So people are altruistic in an even stronger form than needed for an economist's purposes.

    ``J. A. Piliavin and Charng (1990) concluded that: There appears to be a “paradigm shift” away from the earlier position that behavior that appears to be altruistic must, under closer scrutiny, be revealed as reflecting egoistic motives. Rather, theory and data now being advanced are more compatible with the view that true altruism—acting with the goal of benefiting another—does exist and is a part of human nature. (p. 27)''

    Universal principalism seems to be a much weaker foundation for prosocial behaviour (although most moral philosophers since Kant have advocated it). This is good for my model -- it provides a good justification for the network. `Collectivism' (working to benefit one's group) does seem to hold some water as an idea, but is a bit closer to enlightened self-interest. \emph{Approx. 2000 cites.}

    \item \cite{fehr2003nature}: Quite a confusing review article. Worth another read some time. Altruism in humans is a thing. Some/many people both reward good behaviour and punish bad -- both at a cost to themselves. This goes beyond just reputation-based cooperation and reciprocity. \emph{Approx. 4500 cites.}

    \item \cite{fromell2020altruism}: a meta-analysis of 60 experiments (across 22 papers and 12,000+ subjects) on how manipulating subjects towards System 1 (`fast') vs. System 2 (`slow') thinking affects altruism. The bottom line is that the meta-analysis shows a null effect. Altruism may be something that escapes the System 1 -- System 2 divide. Although it's not super clear how to interpret the result. For our model, it's sufficient to note that altruism does generally survive in both systems.
\end{itemize}

\subsection{Internet \& Loneliness}
\begin{itemize}
    \item \cite{kraut1998internet}: 169 people, in 73 households, studies their first 1-2 years online. Finds internet associated with decline in time spent with family and social circle, and increases in depression and loneliness.
\end{itemize}


